Accelerating Sampling and Aggregation Operations in GNN Frameworks with GPU Initiated Direct Storage Accesses

Graph Neural Networks (GNNs) are emerging as a powerful tool for learning from graph-structured data and performing sophisticated inference tasks in various application domains. Although GNNs have been shown to be effective on modest-sized graphs, training them on large-scale graphs remains a significant challenge due to lack of efficient data access and data movement methods. Existing frameworks for training GNNs use CPUs for graph sampling and feature aggregation, while the training and updating of model weights are executed on GPUs. However, our in-depth profiling shows the CPUs cannot achieve the throughput required to saturate GNN model training throughput, causing gross under-utilization of expensive GPU resources. Furthermore, when the graph and its embeddings do not fit in the CPU memory, the overhead introduced by the operating system, say for handling page-faults, comes in the critical path of execution. To address these issues, we propose the GPU Initiated Direct Storage Access (GIDS) dataloader, to enable GPU-oriented GNN training for large-scale graphs while efficiently utilizing all hardware resources, such as CPU memory, storage, and GPU memory with a hybrid data placement strategy. By enabling GPU threads to fetch feature vectors directly from storage, GIDS dataloader solves the memory capacity problem for GPU-oriented GNN training. Moreover, GIDS dataloader leverages GPU parallelism to tolerate storage latency and eliminates expensive page-fault overhead. Doing so enables us to design novel optimizations for exploiting locality and increasing effective bandwidth for GNN training. Our evaluation using a single GPU on terabyte-scale GNN datasets shows that GIDS dataloader accelerates the overall DGL GNN training pipeline by up to 392X when compared to the current, state-of-the-art DGL dataloader.

==> Implementation.tex <==
\section{Implementation}
\zq{this is a very short section, maybe we make it a subsection in another section? what oes everyone think?}
We extended DGL~\cite{dgl}, a popular open-source framework for GNN training, to implement \pname{}. Our approach involves creating new extensions for storage-based feature gathering by leveraging BaM~\cite{bam} to support user-level GPU-initiated direct storage access. We then extended the DGL dataloader class to incorporate \pname{} functionalities. To use the \pname{} dataloader, users only need to set the \pname{} flag when initializing the DGL dataloader. After initializing the dataloader, users can simply call the \pname{} initialization function to set up the controllers for GPU threads storage access and provide information about the location of the node feature data in the SSDs. \zq{why can't this gids initialization just be a part of the datalaoder initialization?}
\bp{I can do that as well. I thought it is more clear than adding 6 additional default parameters for the dataloader initalization}
\zq{what are the 6 additional parameters? can't most of them have defaults? what is the standard way of specializing a dataloader?. There are parameters like offset, cacheline size, number of ssds, number of elements, etc. I can shift them to dataloader initialization, it takes only a few lines of changes.}
Once set up, the \pname{} dataloader can be used in the same way as the DGL dataloader for GNN training, simplifying the process of integrating the \pname{} dataloader into GNN applications.

